Breeze-7B Technical Report

Breeze-7B is an open-source language model based on Mistral-7B, designed to address the need for improved language comprehension and chatbot-oriented capabilities in Traditional Chinese. This technical report provides an overview of the additional pretraining, finetuning, and evaluation stages for the Breeze-7B model. The Breeze-7B family of base and chat models exhibits good performance on language comprehension and chatbot-oriented tasks, reaching the top in several benchmarks among models comparable in its complexity class.

==> finetuning_data.tex <==
\subsubsection{Instruction-tuning Data Selection}
In preliminary experiments, we notice that it is enough to finetune a continuously pretrained model with English finetuning data for activating Chinese chat capability, and that the gain brought by Traditional Chinese supervised finetuning data is trivial. Therefore, we focus on finetuning model with English instruction data.

We list supervised finetuning data in \autoref{table:en_sft_data_collection} and preference finetuning data in \autoref{table:en_preference_data_collection}.


\begin{table}[ht]
  \centering
  \setlength{\tabcolsep}{4pt}
   {
  \begin{tabular}{llr}
    \toprule
     Targeted Capability & Dataset  & \shortstack[r]{Num. of Samples}  \\
     \midrule
     General Chat & SlimOrca & 518 k \\
     General Chat & UltraChat & 200 k \\
     General Chat & ShareGPT & 6.2 k \\
     General Chat & LDJnr/Pure-Dove & 3.8 k \\
     General Chat & OpenAssistant/oasst top1 & 12.9 k \\
     General Chat & WizardLM Evol Instruct & 143 k \\
     STEM         & Camel-AI/Physics & 20 k  \\
     STEM         & Camel-AI/Chemistry & 20 k  \\
     STEM         & Camel-AI/Biology & 20 k  \\
     Math  & Camel-AI/Math & 50 k  \\
     Math  & MetaMathQA & 395 k  \\
     Math  & MathInstruct & 262 k  \\
     Role-play & evol-character-200 (zhsc) & 0.2 k \\
     Role-play & hieunguyenminh/roleplay & 5.7 k \\
     Role-play & Tarklanse/TC roleplay chat (zhtw) & 9.5 k \\
     Coding & evol-codealpaca-v1 & 111k \\
     Coding & glaiveai/glaive-code-assistant & 136 k \\
     General Subjects & GPTeacher & 89.3k\\
     General Subjects & textbook & 682k\\
    \midrule
    Total &  &2584 k \\
    \bottomrule
  \end{tabular}}
  \vspace{0.3cm}
    \caption{\textbf{Statistics of English instruction data for SFT.}} 
  \label{table:en_sft_data_collection}
\end{table}


\begin{table}[ht]
  \centering
  \setlength{\tabcolsep}{4pt}
   {
  \begin{tabular}{llr}
    \toprule
    Targeted Capability & Dataset  & \shortstack[r]{Num. of Samples}  \\
    \midrule
    General Chat & Orca DPO       & 12.9 k \\
                 & Ultra Feedback & 61 k   \\
    Reasoning & ProlificAI/social-reasoning-rlhf & 3.82k \\
    \midrule
    Total &  &77.7 k \\
    \bottomrule
  \end{tabular}}
  \vspace{0.3cm}
    \caption{\textbf{Statistics of English instruction data for SFT.}} 
  \label{table:en_preference_data_collection}
\end{table}

We conduct preliminary experiments to explore the effectiveness of each dataset. To be efficient, we finetune \textbf{STUDENT MODEL} and use \textbf{TEACHER MODEL} as the judge to evaluate fine-tuned model abilities on MT-Bench. We start by using all finetune datasets and remove datasets with negative impact.

==> pretraining_data_collection.tex <==

\subsubsection{Pretraining Data Collection}
For the pretraining data, we both collect raw text via web crawling and use existing Traditional Chinese data. The sources of data are shown in \autoref{table:pretraining_data_sources}. Note that the crawl depth of Taiwanese websites are shallow (reference lost), we additionally targeted multiple Taiwanese large website and crawled the text data more thoroughly.


\begin{table*}[t]
\scriptsize
\begin{tabular}{llll}
\hline
                & Source           & \begin{tabular}[c]{@{}l@{}}Size on Disk\\ (before processing)\end{tabular} & Preprocessing \\ \hline
Taiwan Websites & Web Crawling     & 11.12 GB    & BOF      \\ 
Wiki-zh    & Existing Dataset & 1.01 GB  &   \\
CC-100-zht (from CC 2018 snapshots)  & Existing Dataset & 7.85 GB  & \\ 
C4-zht  (from CC 2018-2020 snapshots)    & Existing Dataset & 8.23 GB &  \\ 
Chinese Poetry  & Collected  &        46 MB     &   \\ 
Taiwan Judicial Data & Collected  &        21.8 GB     &   \\ 
teric.naer & Collected  &        1.4 GB     &   \\ 
GRB & Collected  &  15.5 GB     &   \\ 
Common Crawl   & Existing Dataset &      &  SEO Removal  \\
%-- (2019) (not completed processed)   & Existing Dataset &  3.6 TB  & c4, BOF, SSTC   \\ 
-- (2020-24) (not completed processed)   & Existing Dataset &  144.93 GB  & c4, BOF, SSTC   \\ 
-- (2020-29) (not completed processed)   & Existing Dataset &  145.93 GB  & c4, BOF, SSTC   \\ 
-- (2020-34) (not completed processed)   & Existing Dataset &  119.01 GB  & c4, BOF, SSTC   \\ 
-- (2020-45) (not completed processed)   & Existing Dataset &  124.90 GB  & c4, BOF, SSTC   \\ 
-- (2020-50) (not completed processed)   & Existing Dataset &  110.61 GB  & c4, BOF, SSTC   \\ 
-- (2021-04) (not completed processed)   & Existing Dataset &  128.28 GB  & c4, BOF, SSTC   \\ 
-- (2021-10) (not completed processed)    & Existing Dataset &  109.89 GB & c4, BOF, SSTC   \\ 
-- (2021-21)    & Existing Dataset &  100.14 GB  & SCTCR, c4, BOF   \\ 
-- (2021-25)    & Existing Dataset &  109.23 GB  & SCTCR, c4, BOF   \\ 
-- (2021-31)    & Existing Dataset &  120.83 GB  & SCTCR, c4, BOF   \\ 
-- (2021-39)    & Existing Dataset &  120.40 GB  & SCTCR, c4, BOF   \\ 
-- (2021-43)    & Existing Dataset &  121.74 GB  & SCTCR, c4, BOF   \\ 
-- (2022-05)    & Existing Dataset &  109.87 GB  & SCTCR, c4, BOF   \\ 

-- (2021-49)    & Existing Dataset &  95.93 GB    & cc net, BOF, SSTC   \\ 
-- (2022-21)    & Existing Dataset &  117.02 GB   & cc net, BOF, SSTC   \\ 
-- (2022-27)    & Existing Dataset &  119.12  GB  & cc net, BOF, SSTC   \\ 
-- (2022-33)    & Existing Dataset &  106.76 GB   & cc net, BOF, SSTC   \\ 
-- (2022-40)    & Existing Dataset &  121.28 GB   & cc net, BOF, SSTC   \\ 
-- (2022-49)    & Existing Dataset &  130.13  GB  & cc net, BOF, SSTC   \\ 
-- (2023-06)    & Existing Dataset &  122.39 GB   & cc net, BOF, SSTC   \\ 
-- (2023-14)    & Existing Dataset &  121.21 GB   & cc net, BOF, SSTC   \\ 

Eland Yahoo Knowledge & Purchased & 49.6 GB & BOF \\
Eland Line Q & Purchased & 5.4 GB & BOF \\
Eland Blog & Purchased & 112.7 GB & BOF \\
Eland News & Purchased & 633.0 GB & BOF \\
Eland Forum & Purchased & 177.8 GB & BOF \\
Eland BBS & Purchased & 163.3 GB & BOF \\
\midrule
All             &                  &  3.708 TB  &               \\ \bottomrule
\end{tabular}
    \caption{Source of Traditional Chinese pretraining data. BOF represents the filtering scheme in \citep{scao2022bloom}, cc net represents the processing scheme in \citep{wenzek2020ccnet}, c4 means the processing scheme in \citep{raffel2020exploring}, SSTC means we remove any sample if the sample contain at least single simplified Chinese character. SCTCR means we only keep samples with a traditional Chinese character ratio $>$ 0.2 and a simplified Chinese character ratio $<$ 0.1. 
    Note that the "Size on Disk" of common crawl is referenced from Penny's blog.\footnote{"https://weibo.com/1497035431/NevUys55V"}}
    \label{table:pretraining_data_sources}
\end{table*}



\subsubsection{Pretraining Data Preprocessing}
To optimize the performance of the Language Model (LM), we adopted preprocessing strategies inspired by previous works such as \citep{scao2022bloom} and \citep{wenzek2020ccnet}. For all datasets, we adopted filtering scheme in BLOOM \citep{scao2022bloom}, utilizing the exact parameters delineated in their study.
For content extracted from the Common Crawl dataset, there is additional processing involved. We followed \citep{wenzek2020ccnet}, and isolated Traditional Chinese materials and conducted a deduplication process. To bolster data quality, we eliminated content with perplexity values exceeding 2095 (measured by the language model trained on Wikipedia. See \citep{wenzek2020ccnet}). Furthermore, to mitigate the influence of Simplified Chinese content, we filtered out documents containing Simplified Chinese words.


%\subsubsection{Training Data Composition}
%Our training dataset comprises a blend of 86 GB of Traditional Chinese text.
%and ?GB of English data. The English data have been selectively drawn from Red-pajama\citep{together2023redpajama}. Meanwhile,
%The Traditional Chinese data originate from Common Crawl and have been supplemented with data %obtained through additional web scraping by internal personnel.
%The dataset composition is inspired by previous works such as \citep{penedo2023refinedweb} and \citep{touvron2023llama}. The specific breakdown of this composition is presented in \autoref{table:pretraining_data_makeup}.



==> pretraining_data_composition.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{ l r r }
\textbf{Dataset}           & \textbf{Effective Disk Size} & \textbf{Sampling Weight}       \\
\hline
\textbf{UncommonCrawl}     & 11.9 GB                       & 1.0                     \\
\textbf{CC100~ZHTW}        & 8.4 GB                        & 1.0                    \\
\textbf{Books}             & 1.6 GB                        & 1.0                            \\
\textbf{Thesis}            & 66.6 GB                      & 2.0                            \\
\textbf{Wiki ZH}           & 2.2 GB                        & 2.0                            \\
\textbf{Chinese poetry}    & 0.02 GB                       & 1.0                            \\
\textbf{GRB}               & 23.7 GB                       & 2.0                            \\
\textbf{Judicial}          & 21.4 GB                       & 1.0                            \\
\textbf{Teric.NAER}        & 1.4 GB                        & 1.0                           \\
\textbf{Yamol}             & 0.2 GB                        & 1.0                            \\
\textbf{YouTube subtitles} & 1.1 GB                        & 1.0                            \\
\textbf{C4 ZHTW}           & 8.2 GB                        & 1.0                      \\
\textbf{CommonCrawl}       & 129.2 GB                     & 1.0                           \\
\textbf{LineQA}            & 3.3 GB                       & 1.0                            \\
\textbf{YahooAnswers}      & 14.4 GB                      & 1.0                            \\
\textbf{Blog}              & 36.0 GB                      & 1.0                            \\
\textbf{Github}            & 10.0 GB    & 1.0 \\
\hline\textbf{\textbf{Total}}    & 339.6 GB                      & -                       
\end{tabular}
\caption{The composition of the pretraining data for the additional pretraining stage of M7-D.}
\label{table:data_composition}
\end{table*}
\autoref{table:data_composition} shows the composition of the pretraining dataset.
Talk about composition. Common crawl, thesis, news, programs, ... . 

Talk about selection, in the same way as "textbook is all you need", part 1.

